Is It the Curriculum or Just the Easy Start? Benchmarking Unsupervised Environment Design on Quadrupeds

Unsupervised environment design (UED) methods such as PLR, ACCEL, SFL and PAIRED are compared mostly on 2D mazes, grid worlds and BipedalWalker, while terrain curricula for legged robots are hand-designed and evaluated against a few baselines. We present a benchmark that runs fourteen UED, domain-randomisation and robotics curricula under one protocol on five 3D quadrupeds in MuJoCo MJX: the closed-chain W01-TEK and the open-chain Unitree Go1 and Go2, Google Barkour vB and Boston Dynamics Spot. Levels are vectors of eight interpretable terrain parameters, and all curricula drive the same PPO student at matched environment-step budgets. The evaluation reports success on random and held-out structured terrains, interquartile means with stratified bootstrap intervals, capability envelopes and a level-by-level domination comparison. We compare methods within each robot and report, per level set, the top group of methods not significantly below the best. No method is in the top group on every robot and level set. Methods with easy or low-difficulty training levels, curated or not, fill the top groups on in-distribution random levels of Go1 and Barkour, and of W01-TEK apart from PAIRED+BiBC. The success-driven terrain curriculum from legged-robot practice is in a top group most often, domain randomisation on uniform levels in none, and PAIRED in none outside Spot, where the fourteen methods lie within 3.8 points on random levels of difficulty 0.25. On three robots the leader on in-distribution random levels is not the leader on held-out terrain. We collect the results into a per-robot guide to choosing a curriculum.

==> tables/compute.tex <==
\begin{tabular}{llccc}
\toprule
Robot & Method & GPU-h & Sim steps ($10^6$) & Student steps ($10^6$) \\
\midrule
W01-TEK & DR & 0.5\,{\scriptsize$\pm$0.0} & 302\,{\scriptsize$\pm$0} & 302\,{\scriptsize$\pm$0} \\
 & DR-easy & 0.5\,{\scriptsize$\pm$0.0} & 302\,{\scriptsize$\pm$0} & 302\,{\scriptsize$\pm$0} \\
 & DR-mixed & 0.5\,{\scriptsize$\pm$0.0} & 302\,{\scriptsize$\pm$0} & 302\,{\scriptsize$\pm$0} \\
 & Terrain-CL & 0.5\,{\scriptsize$\pm$0.0} & 302\,{\scriptsize$\pm$0} & 302\,{\scriptsize$\pm$0} \\
 & PLR$^{\perp}$ & 0.5\,{\scriptsize$\pm$0.0} & 302\,{\scriptsize$\pm$0} & 242\,{\scriptsize$\pm$6} \\
 & SFL & 0.5\,{\scriptsize$\pm$0.0} & 302\,{\scriptsize$\pm$0} & 242\,{\scriptsize$\pm$6} \\
 & ACCEL & 0.5\,{\scriptsize$\pm$0.0} & 302\,{\scriptsize$\pm$0} & 229\,{\scriptsize$\pm$6} \\
 & ACCEL-grow & 0.5\,{\scriptsize$\pm$0.0} & 302\,{\scriptsize$\pm$0} & 235\,{\scriptsize$\pm$10} \\
 & ACCEL-SFL & 0.5\,{\scriptsize$\pm$0.0} & 302\,{\scriptsize$\pm$0} & 235\,{\scriptsize$\pm$10} \\
 & ACCEL-LP & 0.5\,{\scriptsize$\pm$0.0} & 302\,{\scriptsize$\pm$0} & 229\,{\scriptsize$\pm$6} \\
 & PAIRED & 0.8\,{\scriptsize$\pm$0.0} & 605\,{\scriptsize$\pm$0} & 302\,{\scriptsize$\pm$0} \\
 & PAIRED+UniBC & 0.9\,{\scriptsize$\pm$0.0} & 605\,{\scriptsize$\pm$0} & 302\,{\scriptsize$\pm$0} \\
 & PAIRED+BiBC & 0.9\,{\scriptsize$\pm$0.0} & 605\,{\scriptsize$\pm$0} & 302\,{\scriptsize$\pm$0} \\
 & PAIRED+Evo & 0.8\,{\scriptsize$\pm$0.0} & 605\,{\scriptsize$\pm$0} & 229\,{\scriptsize$\pm$6} \\
\midrule
Go1 & DR & 0.7\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 1000\,{\scriptsize$\pm$0} \\
 & DR-easy & 0.7\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 1000\,{\scriptsize$\pm$0} \\
 & DR-mixed & 0.7\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 1000\,{\scriptsize$\pm$0} \\
 & Terrain-CL & 0.8\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 1000\,{\scriptsize$\pm$0} \\
 & PLR$^{\perp}$ & 0.7\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 797\,{\scriptsize$\pm$31} \\
 & SFL & 0.7\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 797\,{\scriptsize$\pm$31} \\
 & ACCEL & 0.7\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 786\,{\scriptsize$\pm$19} \\
 & ACCEL-grow & 0.7\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 804\,{\scriptsize$\pm$16} \\
 & ACCEL-SFL & 0.7\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 804\,{\scriptsize$\pm$16} \\
 & ACCEL-LP & 0.7\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 786\,{\scriptsize$\pm$19} \\
 & PAIRED & 1.3\,{\scriptsize$\pm$0.0} & 2000\,{\scriptsize$\pm$0} & 1000\,{\scriptsize$\pm$0} \\
 & PAIRED+UniBC & 1.4\,{\scriptsize$\pm$0.0} & 2000\,{\scriptsize$\pm$0} & 1000\,{\scriptsize$\pm$0} \\
 & PAIRED+BiBC & 1.4\,{\scriptsize$\pm$0.0} & 2000\,{\scriptsize$\pm$0} & 1000\,{\scriptsize$\pm$0} \\
 & PAIRED+Evo & 1.3\,{\scriptsize$\pm$0.0} & 2000\,{\scriptsize$\pm$0} & 786\,{\scriptsize$\pm$19} \\
\midrule
Go2 & DR & 0.9\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 1000\,{\scriptsize$\pm$0} \\
 & DR-easy & 0.9\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 1000\,{\scriptsize$\pm$0} \\
 & DR-mixed & 0.9\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 1000\,{\scriptsize$\pm$0} \\
 & Terrain-CL & 0.9\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 1000\,{\scriptsize$\pm$0} \\
 & PLR$^{\perp}$ & 0.9\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 797\,{\scriptsize$\pm$31} \\
 & SFL & 0.9\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 797\,{\scriptsize$\pm$31} \\
 & ACCEL & 0.9\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 786\,{\scriptsize$\pm$19} \\
 & ACCEL-grow & 0.9\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 804\,{\scriptsize$\pm$16} \\
 & ACCEL-SFL & 0.9\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 804\,{\scriptsize$\pm$16} \\
 & ACCEL-LP & 0.9\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 786\,{\scriptsize$\pm$19} \\
 & PAIRED & 1.6\,{\scriptsize$\pm$0.0} & 2000\,{\scriptsize$\pm$0} & 1000\,{\scriptsize$\pm$0} \\
 & PAIRED+UniBC & 1.7\,{\scriptsize$\pm$0.0} & 2000\,{\scriptsize$\pm$0} & 1000\,{\scriptsize$\pm$0} \\
 & PAIRED+BiBC & 1.7\,{\scriptsize$\pm$0.0} & 2000\,{\scriptsize$\pm$0} & 1000\,{\scriptsize$\pm$0} \\
 & PAIRED+Evo & 1.6\,{\scriptsize$\pm$0.0} & 2000\,{\scriptsize$\pm$0} & 786\,{\scriptsize$\pm$19} \\
\midrule
Barkour vB & DR & 0.8\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 1000\,{\scriptsize$\pm$0} \\
 & DR-easy & 0.8\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 1000\,{\scriptsize$\pm$0} \\
 & DR-mixed & 0.8\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 1000\,{\scriptsize$\pm$0} \\
 & Terrain-CL & 0.8\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 1000\,{\scriptsize$\pm$0} \\
 & PLR$^{\perp}$ & 0.7\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 797\,{\scriptsize$\pm$31} \\
 & SFL & 0.7\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 797\,{\scriptsize$\pm$31} \\
 & ACCEL & 0.7\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 786\,{\scriptsize$\pm$19} \\
 & ACCEL-grow & 0.7\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 804\,{\scriptsize$\pm$16} \\
 & ACCEL-SFL & 0.7\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 804\,{\scriptsize$\pm$16} \\
 & ACCEL-LP & 0.7\,{\scriptsize$\pm$0.0} & 1000\,{\scriptsize$\pm$0} & 786\,{\scriptsize$\pm$19} \\
 & PAIRED & 1.4\,{\scriptsize$\pm$0.0} & 2000\,{\scriptsize$\pm$0} & 1000\,{\scriptsize$\pm$0} \\
 & PAIRED+UniBC & 1.4\,{\scriptsize$\pm$0.0} & 2000\,{\scriptsize$\pm$0} & 1000\,{\scriptsize$\pm$0} \\
 & PAIRED+BiBC & 1.5\,{\scriptsize$\pm$0.0} & 2000\,{\scriptsize$\pm$0} & 1000\,{\scriptsize$\pm$0} \\
 & PAIRED+Evo & 1.3\,{\scriptsize$\pm$0.0} & 2000\,{\scriptsize$\pm$0} & 786\,{\scriptsize$\pm$19} \\
\midrule
Spot & DR & 0.7\,{\scriptsize$\pm$0.0} & 1003\,{\scriptsize$\pm$0} & 1003\,{\scriptsize$\pm$0} \\
 & DR-easy & 0.7\,{\scriptsize$\pm$0.0} & 1003\,{\scriptsize$\pm$0} & 1003\,{\scriptsize$\pm$0} \\
 & DR-mixed & 0.7\,{\scriptsize$\pm$0.0} & 1003\,{\scriptsize$\pm$0} & 1003\,{\scriptsize$\pm$0} \\
 & Terrain-CL & 0.7\,{\scriptsize$\pm$0.0} & 1003\,{\scriptsize$\pm$0} & 1003\,{\scriptsize$\pm$0} \\
 & PLR$^{\perp}$ & 0.7\,{\scriptsize$\pm$0.0} & 1003\,{\scriptsize$\pm$0} & 804\,{\scriptsize$\pm$28} \\
 & SFL & 0.7\,{\scriptsize$\pm$0.0} & 1003\,{\scriptsize$\pm$0} & 804\,{\scriptsize$\pm$28} \\
 & ACCEL & 0.7\,{\scriptsize$\pm$0.0} & 1003\,{\scriptsize$\pm$0} & 764\,{\scriptsize$\pm$23} \\
 & ACCEL-grow & 0.7\,{\scriptsize$\pm$0.0} & 1003\,{\scriptsize$\pm$0} & 788\,{\scriptsize$\pm$28} \\
 & ACCEL-SFL & 0.7\,{\scriptsize$\pm$0.0} & 1003\,{\scriptsize$\pm$0} & 788\,{\scriptsize$\pm$28} \\
 & ACCEL-LP & 0.7\,{\scriptsize$\pm$0.0} & 1003\,{\scriptsize$\pm$0} & 764\,{\scriptsize$\pm$23} \\
 & PAIRED & 1.3\,{\scriptsize$\pm$0.0} & 2006\,{\scriptsize$\pm$0} & 1003\,{\scriptsize$\pm$0} \\
 & PAIRED+UniBC & 1.3\,{\scriptsize$\pm$0.0} & 2006\,{\scriptsize$\pm$0} & 1003\,{\scriptsize$\pm$0} \\
 & PAIRED+BiBC & 1.3\,{\scriptsize$\pm$0.0} & 2006\,{\scriptsize$\pm$0} & 1003\,{\scriptsize$\pm$0} \\
 & PAIRED+Evo & 1.2\,{\scriptsize$\pm$0.0} & 2006\,{\scriptsize$\pm$0} & 764\,{\scriptsize$\pm$23} \\
\bottomrule
\end{tabular}


==> tables/detail.tex <==
\begin{tabular}{llccccc}
\toprule
Robot & Method & $d{=}0.25$ & CVaR$_{25}$ & $d{=}0.5$ & OOD suite & Flat \\
\midrule
W01-TEK & DR & 84.5\,{\scriptsize$\pm$2.4} & 84.6\,{\scriptsize$\pm$2.1} & 75.9\,{\scriptsize$\pm$2.5} & 52.5\,{\scriptsize$\pm$2.1} & 87.3\,{\scriptsize$\pm$1.8} \\
 & DR-easy & 90.2\,{\scriptsize$\pm$0.7} & 89.3\,{\scriptsize$\pm$0.8} & 81.8\,{\scriptsize$\pm$0.8} & 55.4\,{\scriptsize$\pm$0.8} & \textbf{93.7}\,{\scriptsize$\pm$0.5} \\
 & DR-mixed & \textbf{89.9}\,{\scriptsize$\pm$1.1} & \textbf{90.3}\,{\scriptsize$\pm$0.9} & \textbf{83.3}\,{\scriptsize$\pm$1.7} & \textbf{58.5}\,{\scriptsize$\pm$1.0} & 91.9\,{\scriptsize$\pm$1.2} \\
 & Terrain-CL & 87.7\,{\scriptsize$\pm$1.7} & 88.0\,{\scriptsize$\pm$1.4} & 81.8\,{\scriptsize$\pm$1.9} & \textbf{58.9}\,{\scriptsize$\pm$1.3} & 89.6\,{\scriptsize$\pm$1.5} \\
 & PLR$^{\perp}$ & 86.9\,{\scriptsize$\pm$1.4} & 87.0\,{\scriptsize$\pm$1.8} & 78.9\,{\scriptsize$\pm$2.2} & 55.1\,{\scriptsize$\pm$2.0} & 90.0\,{\scriptsize$\pm$1.1} \\
 & SFL & 86.3\,{\scriptsize$\pm$2.1} & 86.4\,{\scriptsize$\pm$2.5} & 79.1\,{\scriptsize$\pm$2.2} & 55.9\,{\scriptsize$\pm$1.3} & 88.4\,{\scriptsize$\pm$1.6} \\
 & ACCEL & \textbf{90.5}\,{\scriptsize$\pm$0.7} & 90.0\,{\scriptsize$\pm$0.6} & \textbf{83.4}\,{\scriptsize$\pm$1.4} & \textbf{57.5}\,{\scriptsize$\pm$1.1} & \textbf{93.8}\,{\scriptsize$\pm$0.4} \\
 & ACCEL-grow & \textbf{91.2}\,{\scriptsize$\pm$0.4} & \textbf{91.2}\,{\scriptsize$\pm$0.4} & \textbf{84.9}\,{\scriptsize$\pm$1.2} & \textbf{59.0}\,{\scriptsize$\pm$1.3} & \textbf{93.4}\,{\scriptsize$\pm$0.2} \\
 & ACCEL-SFL & 83.8\,{\scriptsize$\pm$2.3} & 84.4\,{\scriptsize$\pm$2.5} & 77.8\,{\scriptsize$\pm$1.1} & 54.8\,{\scriptsize$\pm$1.7} & 86.5\,{\scriptsize$\pm$2.7} \\
 & ACCEL-LP & 89.9\,{\scriptsize$\pm$0.6} & 89.2\,{\scriptsize$\pm$0.8} & 81.2\,{\scriptsize$\pm$1.5} & 55.3\,{\scriptsize$\pm$0.7} & \textbf{93.4}\,{\scriptsize$\pm$0.3} \\
 & PAIRED & 81.7\,{\scriptsize$\pm$2.0} & 81.3\,{\scriptsize$\pm$2.1} & 73.8\,{\scriptsize$\pm$1.6} & 50.4\,{\scriptsize$\pm$1.2} & 85.2\,{\scriptsize$\pm$1.1} \\
 & PAIRED+UniBC & 80.5\,{\scriptsize$\pm$2.5} & 80.1\,{\scriptsize$\pm$2.7} & 72.4\,{\scriptsize$\pm$3.0} & 49.5\,{\scriptsize$\pm$2.5} & 84.6\,{\scriptsize$\pm$1.0} \\
 & PAIRED+BiBC & \textbf{70.3}\,{\scriptsize$\pm$26.4} & \textbf{68.8}\,{\scriptsize$\pm$28.0} & \textbf{59.5}\,{\scriptsize$\pm$26.7} & 39.9\,{\scriptsize$\pm$15.3} & \textbf{76.0}\,{\scriptsize$\pm$21.4} \\
 & PAIRED+Evo & 89.2\,{\scriptsize$\pm$1.3} & 89.5\,{\scriptsize$\pm$0.7} & 83.1\,{\scriptsize$\pm$1.0} & \textbf{58.4}\,{\scriptsize$\pm$1.2} & 90.9\,{\scriptsize$\pm$1.8} \\
\midrule
Go1 & DR & 34.9\,{\scriptsize$\pm$4.0} & 27.4\,{\scriptsize$\pm$4.5} & 18.8\,{\scriptsize$\pm$3.4} & 30.2\,{\scriptsize$\pm$2.3} & 65.7\,{\scriptsize$\pm$2.1} \\
 & DR-easy & \textbf{61.6}\,{\scriptsize$\pm$1.9} & 60.4\,{\scriptsize$\pm$2.3} & 46.8\,{\scriptsize$\pm$2.4} & 38.6\,{\scriptsize$\pm$0.9} & \textbf{69.3}\,{\scriptsize$\pm$0.9} \\
 & DR-mixed & \textbf{61.2}\,{\scriptsize$\pm$2.4} & 59.7\,{\scriptsize$\pm$3.1} & \textbf{48.1}\,{\scriptsize$\pm$3.1} & 42.5\,{\scriptsize$\pm$1.2} & \textbf{68.4}\,{\scriptsize$\pm$0.6} \\
 & Terrain-CL & \textbf{62.3}\,{\scriptsize$\pm$2.3} & \textbf{60.9}\,{\scriptsize$\pm$3.1} & \textbf{50.6}\,{\scriptsize$\pm$3.1} & \textbf{45.8}\,{\scriptsize$\pm$0.8} & \textbf{68.6}\,{\scriptsize$\pm$0.7} \\
 & PLR$^{\perp}$ & 45.9\,{\scriptsize$\pm$3.8} & 41.1\,{\scriptsize$\pm$4.3} & 29.8\,{\scriptsize$\pm$4.1} & 38.3\,{\scriptsize$\pm$1.0} & 67.1\,{\scriptsize$\pm$1.1} \\
 & SFL & 45.1\,{\scriptsize$\pm$8.2} & 39.9\,{\scriptsize$\pm$8.4} & 30.6\,{\scriptsize$\pm$7.5} & \textbf{40.5}\,{\scriptsize$\pm$4.4} & \textbf{62.5}\,{\scriptsize$\pm$7.1} \\
 & ACCEL & 53.7\,{\scriptsize$\pm$4.7} & 50.1\,{\scriptsize$\pm$6.3} & 39.3\,{\scriptsize$\pm$6.0} & \textbf{45.1}\,{\scriptsize$\pm$2.1} & \textbf{68.4}\,{\scriptsize$\pm$1.1} \\
 & ACCEL-grow & 49.4\,{\scriptsize$\pm$6.3} & 45.4\,{\scriptsize$\pm$8.0} & 34.2\,{\scriptsize$\pm$6.1} & 42.2\,{\scriptsize$\pm$1.9} & 67.1\,{\scriptsize$\pm$1.5} \\
 & ACCEL-SFL & 57.0\,{\scriptsize$\pm$4.8} & 54.0\,{\scriptsize$\pm$7.2} & 41.8\,{\scriptsize$\pm$5.8} & 41.4\,{\scriptsize$\pm$1.3} & \textbf{69.2}\,{\scriptsize$\pm$0.8} \\
 & ACCEL-LP & \textbf{64.0}\,{\scriptsize$\pm$1.5} & \textbf{63.7}\,{\scriptsize$\pm$2.1} & \textbf{50.8}\,{\scriptsize$\pm$2.3} & 40.4\,{\scriptsize$\pm$1.7} & \textbf{68.9}\,{\scriptsize$\pm$0.8} \\
 & PAIRED & 28.9\,{\scriptsize$\pm$0.9} & 20.5\,{\scriptsize$\pm$0.7} & 15.6\,{\scriptsize$\pm$0.7} & 37.3\,{\scriptsize$\pm$1.9} & \textbf{65.5}\,{\scriptsize$\pm$4.7} \\
 & PAIRED+UniBC & 29.5\,{\scriptsize$\pm$0.6} & 20.4\,{\scriptsize$\pm$0.7} & 16.0\,{\scriptsize$\pm$0.4} & 37.2\,{\scriptsize$\pm$0.8} & 66.7\,{\scriptsize$\pm$1.6} \\
 & PAIRED+BiBC & 24.6\,{\scriptsize$\pm$1.3} & 21.3\,{\scriptsize$\pm$1.2} & 13.7\,{\scriptsize$\pm$1.1} & 21.1\,{\scriptsize$\pm$1.6} & 38.7\,{\scriptsize$\pm$2.2} \\
 & PAIRED+Evo & 33.3\,{\scriptsize$\pm$3.7} & 25.3\,{\scriptsize$\pm$5.0} & 19.1\,{\scriptsize$\pm$2.4} & 40.7\,{\scriptsize$\pm$2.0} & 66.7\,{\scriptsize$\pm$0.9} \\
\midrule
Go2 & DR & 20.0\,{\scriptsize$\pm$8.7} & 15.2\,{\scriptsize$\pm$6.3} & 8.8\,{\scriptsize$\pm$4.0} & 20.4\,{\scriptsize$\pm$9.4} & \textbf{51.2}\,{\scriptsize$\pm$22.7} \\
 & DR-easy & \textbf{33.2}\,{\scriptsize$\pm$6.3} & \textbf{27.1}\,{\scriptsize$\pm$6.9} & \textbf{14.5}\,{\scriptsize$\pm$4.2} & 23.8\,{\scriptsize$\pm$1.9} & \textbf{64.1}\,{\scriptsize$\pm$2.0} \\
 & DR-mixed & 25.9\,{\scriptsize$\pm$1.6} & 19.9\,{\scriptsize$\pm$2.1} & \textbf{12.4}\,{\scriptsize$\pm$1.3} & 27.4\,{\scriptsize$\pm$2.0} & \textbf{62.6}\,{\scriptsize$\pm$1.0} \\
 & Terrain-CL & \textbf{34.1}\,{\scriptsize$\pm$5.2} & \textbf{28.9}\,{\scriptsize$\pm$5.6} & \textbf{17.1}\,{\scriptsize$\pm$4.8} & 27.7\,{\scriptsize$\pm$3.1} & \textbf{63.6}\,{\scriptsize$\pm$1.0} \\
 & PLR$^{\perp}$ & 23.7\,{\scriptsize$\pm$1.0} & 18.3\,{\scriptsize$\pm$1.4} & 10.6\,{\scriptsize$\pm$0.7} & 24.1\,{\scriptsize$\pm$2.0} & \textbf{60.8}\,{\scriptsize$\pm$3.0} \\
 & SFL & \textbf{22.0}\,{\scriptsize$\pm$10.5} & 17.1\,{\scriptsize$\pm$8.0} & \textbf{11.3}\,{\scriptsize$\pm$5.9} & \textbf{24.8}\,{\scriptsize$\pm$12.2} & \textbf{51.2}\,{\scriptsize$\pm$23.9} \\
 & ACCEL & \textbf{27.8}\,{\scriptsize$\pm$2.1} & 21.5\,{\scriptsize$\pm$2.4} & \textbf{15.7}\,{\scriptsize$\pm$1.7} & \textbf{33.4}\,{\scriptsize$\pm$1.5} & \textbf{61.9}\,{\scriptsize$\pm$1.8} \\
 & ACCEL-grow & 24.7\,{\scriptsize$\pm$1.3} & 19.0\,{\scriptsize$\pm$1.4} & \textbf{11.8}\,{\scriptsize$\pm$1.2} & 25.8\,{\scriptsize$\pm$1.7} & 61.4\,{\scriptsize$\pm$1.6} \\
 & ACCEL-SFL & 19.0\,{\scriptsize$\pm$7.9} & 15.0\,{\scriptsize$\pm$4.8} & 9.3\,{\scriptsize$\pm$4.2} & \textbf{22.8}\,{\scriptsize$\pm$11.1} & \textbf{48.2}\,{\scriptsize$\pm$22.9} \\
 & ACCEL-LP & \textbf{28.0}\,{\scriptsize$\pm$12.7} & \textbf{23.4}\,{\scriptsize$\pm$10.6} & \textbf{13.9}\,{\scriptsize$\pm$6.8} & \textbf{23.0}\,{\scriptsize$\pm$9.8} & \textbf{53.0}\,{\scriptsize$\pm$22.3} \\
 & PAIRED & 11.3\,{\scriptsize$\pm$7.4} & 9.8\,{\scriptsize$\pm$5.3} & 4.8\,{\scriptsize$\pm$4.1} & 10.0\,{\scriptsize$\pm$8.0} & 24.9\,{\scriptsize$\pm$17.8} \\
 & PAIRED+UniBC & 10.0\,{\scriptsize$\pm$4.5} & 9.3\,{\scriptsize$\pm$3.9} & 3.7\,{\scriptsize$\pm$2.2} & 7.8\,{\scriptsize$\pm$4.1} & 21.4\,{\scriptsize$\pm$8.7} \\
 & PAIRED+BiBC & 0.2\,{\scriptsize$\pm$0.2} & 0.1\,{\scriptsize$\pm$0.1} & 0.0\,{\scriptsize$\pm$0.0} & 0.1\,{\scriptsize$\pm$0.1} & 0.5\,{\scriptsize$\pm$0.7} \\
 & PAIRED+Evo & 26.3\,{\scriptsize$\pm$4.9} & 20.2\,{\scriptsize$\pm$5.3} & \textbf{13.5}\,{\scriptsize$\pm$3.3} & 29.6\,{\scriptsize$\pm$1.3} & \textbf{63.4}\,{\scriptsize$\pm$2.1} \\
\midrule
Barkour vB & DR & 20.9\,{\scriptsize$\pm$0.9} & 13.4\,{\scriptsize$\pm$0.7} & 7.2\,{\scriptsize$\pm$0.3} & 22.3\,{\scriptsize$\pm$0.8} & 90.9\,{\scriptsize$\pm$0.7} \\
 & DR-easy & \textbf{59.5}\,{\scriptsize$\pm$2.6} & \textbf{48.4}\,{\scriptsize$\pm$4.0} & 20.9\,{\scriptsize$\pm$2.3} & 28.3\,{\scriptsize$\pm$2.0} & \textbf{92.9}\,{\scriptsize$\pm$0.4} \\
 & DR-mixed & 36.4\,{\scriptsize$\pm$2.3} & 25.1\,{\scriptsize$\pm$2.9} & 15.0\,{\scriptsize$\pm$1.5} & 34.2\,{\scriptsize$\pm$2.8} & 92.1\,{\scriptsize$\pm$1.0} \\
 & Terrain-CL & \textbf{60.1}\,{\scriptsize$\pm$1.8} & \textbf{51.9}\,{\scriptsize$\pm$2.1} & \textbf{29.2}\,{\scriptsize$\pm$1.7} & \textbf{42.8}\,{\scriptsize$\pm$3.1} & \textbf{92.6}\,{\scriptsize$\pm$1.1} \\
 & PLR$^{\perp}$ & 33.5\,{\scriptsize$\pm$4.4} & 21.7\,{\scriptsize$\pm$3.7} & 14.8\,{\scriptsize$\pm$2.5} & 37.0\,{\scriptsize$\pm$3.8} & 92.2\,{\scriptsize$\pm$0.9} \\
 & SFL & 31.1\,{\scriptsize$\pm$2.0} & 19.4\,{\scriptsize$\pm$0.7} & 15.5\,{\scriptsize$\pm$0.7} & \textbf{45.2}\,{\scriptsize$\pm$1.5} & \textbf{92.7}\,{\scriptsize$\pm$0.8} \\
 & ACCEL & \textbf{54.7}\,{\scriptsize$\pm$7.2} & \textbf{45.4}\,{\scriptsize$\pm$8.4} & 25.0\,{\scriptsize$\pm$3.4} & 38.3\,{\scriptsize$\pm$1.6} & \textbf{92.7}\,{\scriptsize$\pm$0.8} \\
 & ACCEL-grow & 51.1\,{\scriptsize$\pm$3.2} & 41.1\,{\scriptsize$\pm$3.7} & 24.1\,{\scriptsize$\pm$1.0} & 41.6\,{\scriptsize$\pm$2.3} & \textbf{93.4}\,{\scriptsize$\pm$0.5} \\
 & ACCEL-SFL & \textbf{59.9}\,{\scriptsize$\pm$5.3} & \textbf{51.0}\,{\scriptsize$\pm$6.3} & \textbf{26.1}\,{\scriptsize$\pm$3.8} & 37.2\,{\scriptsize$\pm$3.5} & \textbf{92.9}\,{\scriptsize$\pm$0.5} \\
 & ACCEL-LP & \textbf{59.0}\,{\scriptsize$\pm$4.0} & \textbf{49.2}\,{\scriptsize$\pm$5.5} & 22.2\,{\scriptsize$\pm$3.5} & 30.1\,{\scriptsize$\pm$3.3} & \textbf{92.9}\,{\scriptsize$\pm$0.5} \\
 & PAIRED & 23.0\,{\scriptsize$\pm$0.9} & 14.6\,{\scriptsize$\pm$1.3} & 8.5\,{\scriptsize$\pm$1.0} & 27.1\,{\scriptsize$\pm$1.8} & 89.8\,{\scriptsize$\pm$0.8} \\
 & PAIRED+UniBC & 24.0\,{\scriptsize$\pm$0.9} & 14.6\,{\scriptsize$\pm$1.3} & 8.4\,{\scriptsize$\pm$0.8} & 26.7\,{\scriptsize$\pm$3.8} & 90.2\,{\scriptsize$\pm$0.5} \\
 & PAIRED+BiBC & 27.4\,{\scriptsize$\pm$1.7} & 16.6\,{\scriptsize$\pm$1.4} & 11.7\,{\scriptsize$\pm$0.9} & 35.2\,{\scriptsize$\pm$2.2} & 91.4\,{\scriptsize$\pm$0.5} \\
 & PAIRED+Evo & 25.4\,{\scriptsize$\pm$2.2} & 15.2\,{\scriptsize$\pm$1.7} & 9.0\,{\scriptsize$\pm$2.7} & 32.2\,{\scriptsize$\pm$7.8} & 90.3\,{\scriptsize$\pm$0.3} \\
\midrule
Spot & DR & 14.9\,{\scriptsize$\pm$0.2} & 10.9\,{\scriptsize$\pm$0.6} & 3.1\,{\scriptsize$\pm$0.3} & 9.9\,{\scriptsize$\pm$0.8} & 60.9\,{\scriptsize$\pm$0.5} \\
 & DR-easy & 14.1\,{\scriptsize$\pm$1.1} & 10.3\,{\scriptsize$\pm$0.8} & 2.3\,{\scriptsize$\pm$0.3} & 8.0\,{\scriptsize$\pm$0.8} & 60.8\,{\scriptsize$\pm$0.5} \\
 & DR-mixed & 16.2\,{\scriptsize$\pm$0.4} & 11.6\,{\scriptsize$\pm$0.6} & 3.7\,{\scriptsize$\pm$0.3} & 11.8\,{\scriptsize$\pm$0.7} & 60.4\,{\scriptsize$\pm$0.8} \\
 & Terrain-CL & 16.5\,{\scriptsize$\pm$0.9} & \textbf{11.6}\,{\scriptsize$\pm$0.8} & 3.7\,{\scriptsize$\pm$0.2} & 11.9\,{\scriptsize$\pm$0.5} & \textbf{61.1}\,{\scriptsize$\pm$1.4} \\
 & PLR$^{\perp}$ & 14.3\,{\scriptsize$\pm$1.4} & 10.6\,{\scriptsize$\pm$0.7} & 3.1\,{\scriptsize$\pm$0.7} & 10.2\,{\scriptsize$\pm$1.4} & 60.2\,{\scriptsize$\pm$0.9} \\
 & SFL & 17.0\,{\scriptsize$\pm$0.7} & \textbf{11.9}\,{\scriptsize$\pm$0.7} & 4.7\,{\scriptsize$\pm$0.6} & 15.4\,{\scriptsize$\pm$1.4} & 60.7\,{\scriptsize$\pm$1.1} \\
 & ACCEL & \textbf{17.4}\,{\scriptsize$\pm$0.7} & \textbf{12.5}\,{\scriptsize$\pm$0.2} & 5.5\,{\scriptsize$\pm$0.4} & 17.1\,{\scriptsize$\pm$1.3} & 61.3\,{\scriptsize$\pm$0.9} \\
 & ACCEL-grow & 16.6\,{\scriptsize$\pm$0.6} & \textbf{11.8}\,{\scriptsize$\pm$0.6} & 4.4\,{\scriptsize$\pm$0.7} & 13.8\,{\scriptsize$\pm$1.9} & 60.7\,{\scriptsize$\pm$1.6} \\
 & ACCEL-SFL & \textbf{17.3}\,{\scriptsize$\pm$0.8} & \textbf{12.2}\,{\scriptsize$\pm$0.8} & 4.6\,{\scriptsize$\pm$0.8} & 14.7\,{\scriptsize$\pm$2.0} & 60.4\,{\scriptsize$\pm$1.4} \\
 & ACCEL-LP & 14.8\,{\scriptsize$\pm$1.2} & 10.6\,{\scriptsize$\pm$0.5} & 2.6\,{\scriptsize$\pm$0.5} & 9.0\,{\scriptsize$\pm$1.5} & 61.5\,{\scriptsize$\pm$0.9} \\
 & PAIRED & \textbf{17.6}\,{\scriptsize$\pm$0.5} & \textbf{12.3}\,{\scriptsize$\pm$0.5} & 5.3\,{\scriptsize$\pm$0.6} & 14.9\,{\scriptsize$\pm$1.7} & 61.1\,{\scriptsize$\pm$0.7} \\
 & PAIRED+UniBC & 17.1\,{\scriptsize$\pm$0.3} & \textbf{12.5}\,{\scriptsize$\pm$0.3} & 5.1\,{\scriptsize$\pm$0.3} & 14.7\,{\scriptsize$\pm$1.5} & 60.7\,{\scriptsize$\pm$0.7} \\
 & PAIRED+BiBC & \textbf{17.9}\,{\scriptsize$\pm$0.3} & 11.8\,{\scriptsize$\pm$0.5} & \textbf{7.5}\,{\scriptsize$\pm$0.4} & \textbf{23.2}\,{\scriptsize$\pm$1.6} & \textbf{62.8}\,{\scriptsize$\pm$0.7} \\
 & PAIRED+Evo & \textbf{17.1}\,{\scriptsize$\pm$1.0} & \textbf{12.4}\,{\scriptsize$\pm$0.7} & 5.8\,{\scriptsize$\pm$0.9} & \textbf{21.0}\,{\scriptsize$\pm$2.1} & 60.1\,{\scriptsize$\pm$0.7} \\
\bottomrule
\end{tabular}


==> tables/envelopes.tex <==
\begin{tabular}{llccccccc}
\toprule
Robot & Method & rough (cm) & slope up (deg) & slope down (deg) & stairs up (cm) & stairs down (cm) & gaps (cm) & blocks (cm) \\
\midrule
W01-TEK & DR & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{17.6}\,{\scriptsize$\pm$0.8} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & 4.0\,{\scriptsize$\pm$0.2} & \textbf{8.0}\,{\scriptsize$\pm$0.0} & 5.4\,{\scriptsize$\pm$0.1} & 5.6\,{\scriptsize$\pm$0.2} \\
 & DR-easy & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{18.0}\,{\scriptsize$\pm$0.0} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & 4.6\,{\scriptsize$\pm$0.1} & \textbf{8.0}\,{\scriptsize$\pm$0.0} & 5.5\,{\scriptsize$\pm$0.0} & 5.7\,{\scriptsize$\pm$0.2} \\
 & DR-mixed & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{18.0}\,{\scriptsize$\pm$0.0} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & \textbf{5.0}\,{\scriptsize$\pm$0.0} & \textbf{8.0}\,{\scriptsize$\pm$0.0} & \textbf{5.7}\,{\scriptsize$\pm$0.1} & \textbf{6.0}\,{\scriptsize$\pm$0.0} \\
 & Terrain-CL & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{18.0}\,{\scriptsize$\pm$0.0} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & \textbf{5.0}\,{\scriptsize$\pm$0.0} & \textbf{8.0}\,{\scriptsize$\pm$0.0} & \textbf{5.6}\,{\scriptsize$\pm$0.1} & \textbf{6.0}\,{\scriptsize$\pm$0.0} \\
 & PLR$^{\perp}$ & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{18.0}\,{\scriptsize$\pm$0.0} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & 4.6\,{\scriptsize$\pm$0.3} & \textbf{8.0}\,{\scriptsize$\pm$0.0} & 5.4\,{\scriptsize$\pm$0.1} & \textbf{5.8}\,{\scriptsize$\pm$0.3} \\
 & SFL & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{18.0}\,{\scriptsize$\pm$0.0} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & 4.5\,{\scriptsize$\pm$0.3} & \textbf{8.0}\,{\scriptsize$\pm$0.0} & 5.4\,{\scriptsize$\pm$0.1} & \textbf{6.0}\,{\scriptsize$\pm$0.0} \\
 & ACCEL & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{18.0}\,{\scriptsize$\pm$0.0} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & \textbf{5.0}\,{\scriptsize$\pm$0.0} & \textbf{8.0}\,{\scriptsize$\pm$0.0} & \textbf{5.6}\,{\scriptsize$\pm$0.1} & \textbf{5.9}\,{\scriptsize$\pm$0.1} \\
 & ACCEL-grow & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{18.0}\,{\scriptsize$\pm$0.0} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & \textbf{5.0}\,{\scriptsize$\pm$0.0} & \textbf{8.0}\,{\scriptsize$\pm$0.0} & \textbf{5.7}\,{\scriptsize$\pm$0.2} & \textbf{5.9}\,{\scriptsize$\pm$0.1} \\
 & ACCEL-SFL & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{17.6}\,{\scriptsize$\pm$0.6} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & \textbf{5.0}\,{\scriptsize$\pm$0.0} & \textbf{8.0}\,{\scriptsize$\pm$0.0} & \textbf{5.7}\,{\scriptsize$\pm$0.2} & \textbf{5.8}\,{\scriptsize$\pm$0.2} \\
 & ACCEL-LP & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{18.0}\,{\scriptsize$\pm$0.0} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & 4.7\,{\scriptsize$\pm$0.2} & \textbf{8.0}\,{\scriptsize$\pm$0.0} & 5.5\,{\scriptsize$\pm$0.1} & 5.7\,{\scriptsize$\pm$0.2} \\
 & PAIRED & \textbf{10.0}\,{\scriptsize$\pm$0.0} & 16.5\,{\scriptsize$\pm$1.0} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & 3.8\,{\scriptsize$\pm$0.1} & \textbf{8.0}\,{\scriptsize$\pm$0.0} & 5.4\,{\scriptsize$\pm$0.1} & 5.5\,{\scriptsize$\pm$0.1} \\
 & PAIRED+UniBC & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{15.6}\,{\scriptsize$\pm$2.1} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & 3.8\,{\scriptsize$\pm$0.3} & \textbf{8.0}\,{\scriptsize$\pm$0.0} & 5.3\,{\scriptsize$\pm$0.1} & 5.4\,{\scriptsize$\pm$0.3} \\
 & PAIRED+BiBC & \textbf{8.0}\,{\scriptsize$\pm$4.5} & 9.0\,{\scriptsize$\pm$5.5} & \textbf{16.0}\,{\scriptsize$\pm$8.9} & 2.5\,{\scriptsize$\pm$1.4} & \textbf{6.4}\,{\scriptsize$\pm$3.6} & \textbf{4.3}\,{\scriptsize$\pm$2.4} & \textbf{4.2}\,{\scriptsize$\pm$2.4} \\
 & PAIRED+Evo & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{18.0}\,{\scriptsize$\pm$0.0} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & \textbf{5.0}\,{\scriptsize$\pm$0.0} & \textbf{8.0}\,{\scriptsize$\pm$0.0} & \textbf{5.7}\,{\scriptsize$\pm$0.2} & \textbf{5.9}\,{\scriptsize$\pm$0.1} \\
\midrule
Go1 & DR & \textbf{10.0}\,{\scriptsize$\pm$0.0} & 12.3\,{\scriptsize$\pm$1.9} & \textbf{19.8}\,{\scriptsize$\pm$0.4} & 3.0\,{\scriptsize$\pm$0.3} & 3.7\,{\scriptsize$\pm$0.4} & 0.0\,{\scriptsize$\pm$0.0} & 3.2\,{\scriptsize$\pm$0.2} \\
 & DR-easy & \textbf{10.0}\,{\scriptsize$\pm$0.0} & 16.5\,{\scriptsize$\pm$0.9} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & 3.5\,{\scriptsize$\pm$0.1} & 6.1\,{\scriptsize$\pm$0.6} & \textbf{2.1}\,{\scriptsize$\pm$0.4} & 3.5\,{\scriptsize$\pm$0.1} \\
 & DR-mixed & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{18.0}\,{\scriptsize$\pm$0.0} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & 3.8\,{\scriptsize$\pm$0.1} & 7.0\,{\scriptsize$\pm$0.4} & 2.0\,{\scriptsize$\pm$0.4} & 3.7\,{\scriptsize$\pm$0.1} \\
 & Terrain-CL & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{18.0}\,{\scriptsize$\pm$0.0} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & \textbf{4.1}\,{\scriptsize$\pm$0.2} & \textbf{7.7}\,{\scriptsize$\pm$0.4} & \textbf{2.1}\,{\scriptsize$\pm$0.5} & \textbf{4.0}\,{\scriptsize$\pm$0.2} \\
 & PLR$^{\perp}$ & \textbf{10.0}\,{\scriptsize$\pm$0.0} & 15.4\,{\scriptsize$\pm$0.6} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & 3.5\,{\scriptsize$\pm$0.1} & 5.7\,{\scriptsize$\pm$0.4} & 0.0\,{\scriptsize$\pm$0.0} & \textbf{3.8}\,{\scriptsize$\pm$0.2} \\
 & SFL & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{17.6}\,{\scriptsize$\pm$0.9} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & \textbf{3.6}\,{\scriptsize$\pm$0.6} & 6.6\,{\scriptsize$\pm$0.7} & 0.2\,{\scriptsize$\pm$0.5} & \textbf{3.5}\,{\scriptsize$\pm$0.5} \\
 & ACCEL & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{18.0}\,{\scriptsize$\pm$0.0} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & \textbf{3.9}\,{\scriptsize$\pm$0.4} & \textbf{7.8}\,{\scriptsize$\pm$0.2} & 0.8\,{\scriptsize$\pm$0.8} & \textbf{4.0}\,{\scriptsize$\pm$0.3} \\
 & ACCEL-grow & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{18.0}\,{\scriptsize$\pm$0.0} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & 3.7\,{\scriptsize$\pm$0.2} & 6.6\,{\scriptsize$\pm$0.6} & 0.4\,{\scriptsize$\pm$0.6} & \textbf{3.8}\,{\scriptsize$\pm$0.4} \\
 & ACCEL-SFL & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{17.6}\,{\scriptsize$\pm$0.5} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & 3.5\,{\scriptsize$\pm$0.1} & \textbf{7.5}\,{\scriptsize$\pm$0.5} & 1.4\,{\scriptsize$\pm$0.5} & 3.5\,{\scriptsize$\pm$0.1} \\
 & ACCEL-LP & \textbf{10.0}\,{\scriptsize$\pm$0.0} & 16.3\,{\scriptsize$\pm$1.1} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & 3.5\,{\scriptsize$\pm$0.1} & \textbf{7.2}\,{\scriptsize$\pm$0.7} & \textbf{2.7}\,{\scriptsize$\pm$0.5} & 3.5\,{\scriptsize$\pm$0.1} \\
 & PAIRED & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{16.9}\,{\scriptsize$\pm$1.1} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & 3.6\,{\scriptsize$\pm$0.2} & 4.7\,{\scriptsize$\pm$0.1} & 0.0\,{\scriptsize$\pm$0.0} & 3.5\,{\scriptsize$\pm$0.1} \\
 & PAIRED+UniBC & \textbf{10.0}\,{\scriptsize$\pm$0.0} & 16.8\,{\scriptsize$\pm$0.7} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & 3.6\,{\scriptsize$\pm$0.1} & 4.7\,{\scriptsize$\pm$0.1} & 0.0\,{\scriptsize$\pm$0.0} & 3.5\,{\scriptsize$\pm$0.1} \\
 & PAIRED+BiBC & 0.0\,{\scriptsize$\pm$0.0} & 0.0\,{\scriptsize$\pm$0.0} & 0.0\,{\scriptsize$\pm$0.0} & 0.0\,{\scriptsize$\pm$0.0} & 0.0\,{\scriptsize$\pm$0.0} & 0.0\,{\scriptsize$\pm$0.0} & 0.0\,{\scriptsize$\pm$0.0} \\
 & PAIRED+Evo & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{18.0}\,{\scriptsize$\pm$0.0} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & 3.4\,{\scriptsize$\pm$0.3} & 6.0\,{\scriptsize$\pm$0.6} & 0.0\,{\scriptsize$\pm$0.0} & 3.5\,{\scriptsize$\pm$0.2} \\
\midrule
Go2 & DR & \textbf{7.9}\,{\scriptsize$\pm$4.4} & \textbf{8.9}\,{\scriptsize$\pm$5.2} & 11.0\,{\scriptsize$\pm$6.3} & \textbf{1.6}\,{\scriptsize$\pm$0.9} & 2.3\,{\scriptsize$\pm$1.3} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & \textbf{2.1}\,{\scriptsize$\pm$1.2} \\
 & DR-easy & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{11.8}\,{\scriptsize$\pm$0.9} & 15.8\,{\scriptsize$\pm$2.6} & 1.8\,{\scriptsize$\pm$0.1} & 2.7\,{\scriptsize$\pm$0.5} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & 2.2\,{\scriptsize$\pm$0.2} \\
 & DR-mixed & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{12.8}\,{\scriptsize$\pm$0.3} & \textbf{19.1}\,{\scriptsize$\pm$1.1} & 2.0\,{\scriptsize$\pm$0.2} & 3.5\,{\scriptsize$\pm$0.3} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & 2.6\,{\scriptsize$\pm$0.3} \\
 & Terrain-CL & \textbf{10.0}\,{\scriptsize$\pm$0.0} & 11.7\,{\scriptsize$\pm$0.9} & \textbf{18.3}\,{\scriptsize$\pm$1.4} & \textbf{2.3}\,{\scriptsize$\pm$0.5} & 3.4\,{\scriptsize$\pm$0.5} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & \textbf{2.6}\,{\scriptsize$\pm$0.5} \\
 & PLR$^{\perp}$ & \textbf{9.6}\,{\scriptsize$\pm$0.6} & \textbf{10.0}\,{\scriptsize$\pm$3.8} & 14.0\,{\scriptsize$\pm$2.5} & 2.0\,{\scriptsize$\pm$0.1} & 2.9\,{\scriptsize$\pm$0.2} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & 2.4\,{\scriptsize$\pm$0.2} \\
 & SFL & \textbf{8.0}\,{\scriptsize$\pm$4.5} & \textbf{10.2}\,{\scriptsize$\pm$6.2} & \textbf{15.9}\,{\scriptsize$\pm$8.9} & \textbf{1.8}\,{\scriptsize$\pm$1.0} & 3.2\,{\scriptsize$\pm$1.8} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & \textbf{2.2}\,{\scriptsize$\pm$1.3} \\
 & ACCEL & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{12.4}\,{\scriptsize$\pm$2.2} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & \textbf{2.4}\,{\scriptsize$\pm$0.3} & \textbf{5.8}\,{\scriptsize$\pm$1.0} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & \textbf{3.2}\,{\scriptsize$\pm$0.3} \\
 & ACCEL-grow & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{11.3}\,{\scriptsize$\pm$1.3} & 16.7\,{\scriptsize$\pm$1.9} & 2.0\,{\scriptsize$\pm$0.2} & 3.1\,{\scriptsize$\pm$0.8} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & 2.4\,{\scriptsize$\pm$0.3} \\
 & ACCEL-SFL & \textbf{6.0}\,{\scriptsize$\pm$5.5} & \textbf{8.3}\,{\scriptsize$\pm$7.6} & \textbf{12.0}\,{\scriptsize$\pm$11.0} & \textbf{1.2}\,{\scriptsize$\pm$1.1} & 2.5\,{\scriptsize$\pm$2.3} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & \textbf{1.6}\,{\scriptsize$\pm$1.5} \\
 & ACCEL-LP & \textbf{8.0}\,{\scriptsize$\pm$4.5} & \textbf{8.9}\,{\scriptsize$\pm$5.1} & \textbf{15.2}\,{\scriptsize$\pm$8.5} & \textbf{1.9}\,{\scriptsize$\pm$1.1} & 2.7\,{\scriptsize$\pm$1.5} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & \textbf{2.2}\,{\scriptsize$\pm$1.3} \\
 & PAIRED & 1.6\,{\scriptsize$\pm$3.6} & 1.3\,{\scriptsize$\pm$2.9} & 3.3\,{\scriptsize$\pm$7.4} & 0.4\,{\scriptsize$\pm$0.8} & 0.7\,{\scriptsize$\pm$1.6} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & 0.5\,{\scriptsize$\pm$1.0} \\
 & PAIRED+UniBC & 0.0\,{\scriptsize$\pm$0.0} & 0.0\,{\scriptsize$\pm$0.0} & 0.0\,{\scriptsize$\pm$0.0} & 0.0\,{\scriptsize$\pm$0.0} & 0.0\,{\scriptsize$\pm$0.0} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & 0.0\,{\scriptsize$\pm$0.0} \\
 & PAIRED+BiBC & 0.0\,{\scriptsize$\pm$0.0} & 0.0\,{\scriptsize$\pm$0.0} & 0.0\,{\scriptsize$\pm$0.0} & 0.0\,{\scriptsize$\pm$0.0} & 0.0\,{\scriptsize$\pm$0.0} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & 0.0\,{\scriptsize$\pm$0.0} \\
 & PAIRED+Evo & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{12.1}\,{\scriptsize$\pm$2.0} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & \textbf{2.0}\,{\scriptsize$\pm$0.5} & \textbf{4.8}\,{\scriptsize$\pm$0.5} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & \textbf{2.6}\,{\scriptsize$\pm$0.5} \\
\midrule
Barkour vB & DR & 7.8\,{\scriptsize$\pm$0.5} & 14.1\,{\scriptsize$\pm$0.7} & 8.5\,{\scriptsize$\pm$0.7} & 3.1\,{\scriptsize$\pm$0.2} & 2.3\,{\scriptsize$\pm$0.1} & 0.0\,{\scriptsize$\pm$0.0} & 2.2\,{\scriptsize$\pm$0.1} \\
 & DR-easy & \textbf{9.9}\,{\scriptsize$\pm$0.2} & 13.8\,{\scriptsize$\pm$0.8} & 11.5\,{\scriptsize$\pm$0.8} & 3.5\,{\scriptsize$\pm$0.1} & 3.3\,{\scriptsize$\pm$0.2} & \textbf{1.5}\,{\scriptsize$\pm$0.0} & 3.0\,{\scriptsize$\pm$0.2} \\
 & DR-mixed & \textbf{10.0}\,{\scriptsize$\pm$0.0} & 16.5\,{\scriptsize$\pm$1.0} & 14.9\,{\scriptsize$\pm$1.1} & 3.4\,{\scriptsize$\pm$0.3} & 3.7\,{\scriptsize$\pm$0.2} & 0.0\,{\scriptsize$\pm$0.0} & 3.1\,{\scriptsize$\pm$0.3} \\
 & Terrain-CL & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{17.8}\,{\scriptsize$\pm$0.3} & \textbf{19.3}\,{\scriptsize$\pm$0.7} & 3.9\,{\scriptsize$\pm$0.2} & \textbf{4.9}\,{\scriptsize$\pm$0.3} & 1.4\,{\scriptsize$\pm$0.0} & 3.7\,{\scriptsize$\pm$0.2} \\
 & PLR$^{\perp}$ & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{17.0}\,{\scriptsize$\pm$1.0} & 16.4\,{\scriptsize$\pm$1.6} & 3.8\,{\scriptsize$\pm$0.2} & 4.0\,{\scriptsize$\pm$0.4} & 0.0\,{\scriptsize$\pm$0.0} & 3.5\,{\scriptsize$\pm$0.2} \\
 & SFL & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{18.0}\,{\scriptsize$\pm$0.0} & \textbf{18.5}\,{\scriptsize$\pm$0.8} & \textbf{4.4}\,{\scriptsize$\pm$0.1} & \textbf{4.8}\,{\scriptsize$\pm$0.5} & 0.0\,{\scriptsize$\pm$0.0} & \textbf{4.0}\,{\scriptsize$\pm$0.2} \\
 & ACCEL & \textbf{10.0}\,{\scriptsize$\pm$0.0} & 14.1\,{\scriptsize$\pm$0.9} & \textbf{18.6}\,{\scriptsize$\pm$1.0} & 3.5\,{\scriptsize$\pm$0.1} & \textbf{5.0}\,{\scriptsize$\pm$0.3} & \textbf{1.0}\,{\scriptsize$\pm$0.6} & 3.5\,{\scriptsize$\pm$0.1} \\
 & ACCEL-grow & \textbf{10.0}\,{\scriptsize$\pm$0.0} & 16.1\,{\scriptsize$\pm$1.4} & \textbf{19.1}\,{\scriptsize$\pm$1.0} & 3.7\,{\scriptsize$\pm$0.2} & \textbf{5.3}\,{\scriptsize$\pm$0.5} & 0.7\,{\scriptsize$\pm$0.6} & 3.6\,{\scriptsize$\pm$0.2} \\
 & ACCEL-SFL & \textbf{10.0}\,{\scriptsize$\pm$0.0} & \textbf{17.1}\,{\scriptsize$\pm$1.1} & 15.7\,{\scriptsize$\pm$2.1} & 3.8\,{\scriptsize$\pm$0.3} & 4.4\,{\scriptsize$\pm$0.5} & \textbf{1.4}\,{\scriptsize$\pm$0.2} & 3.5\,{\scriptsize$\pm$0.2} \\
 & ACCEL-LP & \textbf{9.9}\,{\scriptsize$\pm$0.2} & 13.7\,{\scriptsize$\pm$1.2} & 12.8\,{\scriptsize$\pm$2.1} & 3.5\,{\scriptsize$\pm$0.1} & 3.6\,{\scriptsize$\pm$0.4} & \textbf{1.5}\,{\scriptsize$\pm$0.1} & 3.1\,{\scriptsize$\pm$0.2} \\
 & PAIRED & \textbf{9.7}\,{\scriptsize$\pm$0.3} & 12.9\,{\scriptsize$\pm$2.1} & 11.2\,{\scriptsize$\pm$0.6} & 3.0\,{\scriptsize$\pm$0.2} & 3.2\,{\scriptsize$\pm$0.2} & 0.0\,{\scriptsize$\pm$0.0} & 2.9\,{\scriptsize$\pm$0.2} \\
 & PAIRED+UniBC & 9.0\,{\scriptsize$\pm$0.7} & \textbf{14.3}\,{\scriptsize$\pm$3.1} & 10.1\,{\scriptsize$\pm$1.8} & 3.4\,{\scriptsize$\pm$0.5} & 3.0\,{\scriptsize$\pm$0.3} & 0.0\,{\scriptsize$\pm$0.0} & 2.7\,{\scriptsize$\pm$0.2} \\
 & PAIRED+BiBC & \textbf{10.0}\,{\scriptsize$\pm$0.0} & 13.9\,{\scriptsize$\pm$1.9} & 14.8\,{\scriptsize$\pm$1.6} & 3.2\,{\scriptsize$\pm$0.1} & 4.0\,{\scriptsize$\pm$0.3} & 0.0\,{\scriptsize$\pm$0.0} & 3.4\,{\scriptsize$\pm$0.2} \\
 & PAIRED+Evo & \textbf{9.0}\,{\scriptsize$\pm$1.2} & \textbf{17.8}\,{\scriptsize$\pm$0.5} & 11.5\,{\scriptsize$\pm$5.3} & \textbf{4.0}\,{\scriptsize$\pm$0.9} & 3.1\,{\scriptsize$\pm$0.8} & 0.0\,{\scriptsize$\pm$0.0} & 2.9\,{\scriptsize$\pm$0.4} \\
\midrule
Spot & DR & 5.5\,{\scriptsize$\pm$0.1} & 0.0\,{\scriptsize$\pm$0.0} & 9.1\,{\scriptsize$\pm$0.6} & 0.5\,{\scriptsize$\pm$0.5} & 1.6\,{\scriptsize$\pm$0.1} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & 1.2\,{\scriptsize$\pm$0.0} \\
 & DR-easy & 5.2\,{\scriptsize$\pm$0.4} & 0.0\,{\scriptsize$\pm$0.0} & 8.4\,{\scriptsize$\pm$0.5} & \textbf{0.6}\,{\scriptsize$\pm$0.5} & 1.2\,{\scriptsize$\pm$0.7} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & 0.9\,{\scriptsize$\pm$0.5} \\
 & DR-mixed & 5.9\,{\scriptsize$\pm$0.1} & 0.0\,{\scriptsize$\pm$0.0} & 10.6\,{\scriptsize$\pm$0.7} & 0.7\,{\scriptsize$\pm$0.4} & 1.6\,{\scriptsize$\pm$0.0} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & 1.2\,{\scriptsize$\pm$0.0} \\
 & Terrain-CL & 6.0\,{\scriptsize$\pm$0.1} & 0.7\,{\scriptsize$\pm$1.6} & 11.2\,{\scriptsize$\pm$0.8} & 0.9\,{\scriptsize$\pm$0.0} & 1.6\,{\scriptsize$\pm$0.0} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & 1.2\,{\scriptsize$\pm$0.0} \\
 & PLR$^{\perp}$ & 5.4\,{\scriptsize$\pm$0.2} & 0.0\,{\scriptsize$\pm$0.0} & 10.0\,{\scriptsize$\pm$0.8} & 0.3\,{\scriptsize$\pm$0.5} & 0.9\,{\scriptsize$\pm$0.9} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & 0.9\,{\scriptsize$\pm$0.5} \\
 & SFL & 6.6\,{\scriptsize$\pm$0.5} & \textbf{3.0}\,{\scriptsize$\pm$1.9} & 13.9\,{\scriptsize$\pm$2.3} & 1.0\,{\scriptsize$\pm$0.1} & 1.7\,{\scriptsize$\pm$0.1} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & 1.3\,{\scriptsize$\pm$0.1} \\
 & ACCEL & 6.7\,{\scriptsize$\pm$1.1} & 2.2\,{\scriptsize$\pm$2.1} & 15.4\,{\scriptsize$\pm$0.8} & 1.0\,{\scriptsize$\pm$0.1} & 2.0\,{\scriptsize$\pm$0.2} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & 1.3\,{\scriptsize$\pm$0.1} \\
 & ACCEL-grow & 6.1\,{\scriptsize$\pm$0.3} & 0.6\,{\scriptsize$\pm$1.4} & 12.7\,{\scriptsize$\pm$2.2} & 0.9\,{\scriptsize$\pm$0.0} & 1.7\,{\scriptsize$\pm$0.1} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & 1.3\,{\scriptsize$\pm$0.1} \\
 & ACCEL-SFL & 6.2\,{\scriptsize$\pm$0.6} & 1.6\,{\scriptsize$\pm$2.2} & 12.8\,{\scriptsize$\pm$1.2} & \textbf{0.8}\,{\scriptsize$\pm$0.4} & 1.8\,{\scriptsize$\pm$0.3} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & 1.3\,{\scriptsize$\pm$0.1} \\
 & ACCEL-LP & 5.6\,{\scriptsize$\pm$0.1} & 0.7\,{\scriptsize$\pm$1.6} & 8.7\,{\scriptsize$\pm$1.0} & 0.9\,{\scriptsize$\pm$0.1} & 1.6\,{\scriptsize$\pm$0.1} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & 1.2\,{\scriptsize$\pm$0.0} \\
 & PAIRED & 6.2\,{\scriptsize$\pm$0.3} & 0.0\,{\scriptsize$\pm$0.0} & 12.2\,{\scriptsize$\pm$1.3} & 0.9\,{\scriptsize$\pm$0.1} & 1.9\,{\scriptsize$\pm$0.1} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & 1.4\,{\scriptsize$\pm$0.1} \\
 & PAIRED+UniBC & 6.2\,{\scriptsize$\pm$0.4} & 0.0\,{\scriptsize$\pm$0.0} & 12.3\,{\scriptsize$\pm$1.0} & 0.9\,{\scriptsize$\pm$0.0} & 1.8\,{\scriptsize$\pm$0.1} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & 1.3\,{\scriptsize$\pm$0.1} \\
 & PAIRED+BiBC & \textbf{9.0}\,{\scriptsize$\pm$0.3} & \textbf{5.2}\,{\scriptsize$\pm$0.8} & \textbf{19.3}\,{\scriptsize$\pm$1.2} & \textbf{1.2}\,{\scriptsize$\pm$0.1} & \textbf{2.7}\,{\scriptsize$\pm$0.3} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & \textbf{1.8}\,{\scriptsize$\pm$0.1} \\
 & PAIRED+Evo & 5.9\,{\scriptsize$\pm$0.4} & 0.0\,{\scriptsize$\pm$0.0} & \textbf{20.0}\,{\scriptsize$\pm$0.0} & 0.5\,{\scriptsize$\pm$0.5} & 2.0\,{\scriptsize$\pm$0.4} & \textbf{0.0}\,{\scriptsize$\pm$0.0} & 1.2\,{\scriptsize$\pm$0.2} \\
\bottomrule
\end{tabular}


==> tables/guide.tex <==
\begin{tabular}{l cccc cccc cccc cccc cccc}
\toprule
 & \multicolumn{4}{c}{W01-TEK} & \multicolumn{4}{c}{Go1} & \multicolumn{4}{c}{Go2} & \multicolumn{4}{c}{Barkour vB} & \multicolumn{4}{c}{Spot} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}\cmidrule(lr){14-17}\cmidrule(lr){18-21}
Method & $.25$ & $.5$ & OOD & U & $.25$ & $.5$ & OOD & U & $.25$ & $.5$ & OOD & U & $.25$ & $.5$ & OOD & U & $.25$ & $.5$ & OOD & U \\
\midrule
DR &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
DR-easy &  &  &  &  & $\bullet$ &  &  &  & $\bullet$ & $\bullet$ &  &  & $\bullet$ &  &  &  &  &  &  &  \\
DR-mixed & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &  &  &  & $\bullet$ &  &  &  &  &  &  &  &  &  &  \\
Terrain-CL &  &  & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &  & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &  &  &  &  \\
PLR$^{\perp}$ &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
SFL &  &  &  &  &  &  & $\bullet$ &  & $\bullet$ & $\bullet$ & $\bullet$ &  &  &  & $\bullet$ &  &  &  &  &  \\
ACCEL & $\bullet$ & $\bullet$ & $\bullet$ &  &  &  & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &  &  &  & $\bullet$ &  &  &  \\
ACCEL-grow & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &  &  &  &  &  & $\bullet$ &  &  &  &  &  &  &  &  &  &  \\
ACCEL-SFL &  &  &  &  &  &  &  &  &  &  & $\bullet$ &  & $\bullet$ & $\bullet$ &  &  & $\bullet$ &  &  &  \\
ACCEL-LP &  &  &  &  & $\bullet$ & $\bullet$ &  & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ &  & $\bullet$ &  &  &  &  &  &  &  \\
PAIRED &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  & $\bullet$ &  &  &  \\
PAIRED+UniBC &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  &  \\
PAIRED+BiBC & $\bullet$ & $\bullet$ &  & $\bullet$ &  &  &  &  &  &  &  &  &  &  &  &  & $\bullet$ & $\bullet$ & $\bullet$ & $\bullet$ \\
PAIRED+Evo &  &  & $\bullet$ & $\bullet$ &  &  &  &  &  & $\bullet$ &  &  &  &  &  &  & $\bullet$ &  & $\bullet$ &  \\
\bottomrule
\end{tabular}


==> tables/main.tex <==
\begin{tabular}{lcc cc cc cc cc}
\toprule
 & \multicolumn{2}{c}{W01-TEK} & \multicolumn{2}{c}{Go1} & \multicolumn{2}{c}{Go2} & \multicolumn{2}{c}{Barkour vB} & \multicolumn{2}{c}{Spot} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}\cmidrule(lr){10-11}
Method & $d{=}0.25$ & OOD suite & $d{=}0.25$ & OOD suite & $d{=}0.25$ & OOD suite & $d{=}0.25$ & OOD suite & $d{=}0.25$ & OOD suite \\
\midrule
DR & 84.5\,{\scriptsize$\pm$2.4} & 52.5\,{\scriptsize$\pm$2.1} & 34.9\,{\scriptsize$\pm$4.0} & 30.2\,{\scriptsize$\pm$2.3} & 20.0\,{\scriptsize$\pm$8.7} & 20.4\,{\scriptsize$\pm$9.4} & 20.9\,{\scriptsize$\pm$0.9} & 22.3\,{\scriptsize$\pm$0.8} & 14.9\,{\scriptsize$\pm$0.2} & 9.9\,{\scriptsize$\pm$0.8} \\
DR-easy & 90.2\,{\scriptsize$\pm$0.7} & 55.4\,{\scriptsize$\pm$0.8} & \textbf{61.6}\,{\scriptsize$\pm$1.9} & 38.6\,{\scriptsize$\pm$0.9} & \textbf{33.2}\,{\scriptsize$\pm$6.3} & 23.8\,{\scriptsize$\pm$1.9} & \textbf{59.5}\,{\scriptsize$\pm$2.6} & 28.3\,{\scriptsize$\pm$2.0} & 14.1\,{\scriptsize$\pm$1.1} & 8.0\,{\scriptsize$\pm$0.8} \\
DR-mixed & \textbf{89.9}\,{\scriptsize$\pm$1.1} & \textbf{58.5}\,{\scriptsize$\pm$1.0} & \textbf{61.2}\,{\scriptsize$\pm$2.4} & 42.5\,{\scriptsize$\pm$1.2} & 25.9\,{\scriptsize$\pm$1.6} & 27.4\,{\scriptsize$\pm$2.0} & 36.4\,{\scriptsize$\pm$2.3} & 34.2\,{\scriptsize$\pm$2.8} & 16.2\,{\scriptsize$\pm$0.4} & 11.8\,{\scriptsize$\pm$0.7} \\
Terrain-CL & 87.7\,{\scriptsize$\pm$1.7} & \textbf{58.9}\,{\scriptsize$\pm$1.3} & \textbf{62.3}\,{\scriptsize$\pm$2.3} & \textbf{45.8}\,{\scriptsize$\pm$0.8} & \textbf{34.1}\,{\scriptsize$\pm$5.2} & 27.7\,{\scriptsize$\pm$3.1} & \textbf{60.1}\,{\scriptsize$\pm$1.8} & \textbf{42.8}\,{\scriptsize$\pm$3.1} & 16.5\,{\scriptsize$\pm$0.9} & 11.9\,{\scriptsize$\pm$0.5} \\
PLR$^{\perp}$ & 86.9\,{\scriptsize$\pm$1.4} & 55.1\,{\scriptsize$\pm$2.0} & 45.9\,{\scriptsize$\pm$3.8} & 38.3\,{\scriptsize$\pm$1.0} & 23.7\,{\scriptsize$\pm$1.0} & 24.1\,{\scriptsize$\pm$2.0} & 33.5\,{\scriptsize$\pm$4.4} & 37.0\,{\scriptsize$\pm$3.8} & 14.3\,{\scriptsize$\pm$1.4} & 10.2\,{\scriptsize$\pm$1.4} \\
SFL & 86.3\,{\scriptsize$\pm$2.1} & 55.9\,{\scriptsize$\pm$1.3} & 45.1\,{\scriptsize$\pm$8.2} & \textbf{40.5}\,{\scriptsize$\pm$4.4} & \textbf{22.0}\,{\scriptsize$\pm$10.5} & \textbf{24.8}\,{\scriptsize$\pm$12.2} & 31.1\,{\scriptsize$\pm$2.0} & \textbf{45.2}\,{\scriptsize$\pm$1.5} & 17.0\,{\scriptsize$\pm$0.7} & 15.4\,{\scriptsize$\pm$1.4} \\
ACCEL & \textbf{90.5}\,{\scriptsize$\pm$0.7} & \textbf{57.5}\,{\scriptsize$\pm$1.1} & 53.7\,{\scriptsize$\pm$4.7} & \textbf{45.1}\,{\scriptsize$\pm$2.1} & \textbf{27.8}\,{\scriptsize$\pm$2.1} & \textbf{33.4}\,{\scriptsize$\pm$1.5} & \textbf{54.7}\,{\scriptsize$\pm$7.2} & 38.3\,{\scriptsize$\pm$1.6} & \textbf{17.4}\,{\scriptsize$\pm$0.7} & 17.1\,{\scriptsize$\pm$1.3} \\
ACCEL-grow & \textbf{91.2}\,{\scriptsize$\pm$0.4} & \textbf{59.0}\,{\scriptsize$\pm$1.3} & 49.4\,{\scriptsize$\pm$6.3} & 42.2\,{\scriptsize$\pm$1.9} & 24.7\,{\scriptsize$\pm$1.3} & 25.8\,{\scriptsize$\pm$1.7} & 51.1\,{\scriptsize$\pm$3.2} & 41.6\,{\scriptsize$\pm$2.3} & 16.6\,{\scriptsize$\pm$0.6} & 13.8\,{\scriptsize$\pm$1.9} \\
ACCEL-SFL & 83.8\,{\scriptsize$\pm$2.3} & 54.8\,{\scriptsize$\pm$1.7} & 57.0\,{\scriptsize$\pm$4.8} & 41.4\,{\scriptsize$\pm$1.3} & 19.0\,{\scriptsize$\pm$7.9} & \textbf{22.8}\,{\scriptsize$\pm$11.1} & \textbf{59.9}\,{\scriptsize$\pm$5.3} & 37.2\,{\scriptsize$\pm$3.5} & \textbf{17.3}\,{\scriptsize$\pm$0.8} & 14.7\,{\scriptsize$\pm$2.0} \\
ACCEL-LP & 89.9\,{\scriptsize$\pm$0.6} & 55.3\,{\scriptsize$\pm$0.7} & \textbf{64.0}\,{\scriptsize$\pm$1.5} & 40.4\,{\scriptsize$\pm$1.7} & \textbf{28.0}\,{\scriptsize$\pm$12.7} & \textbf{23.0}\,{\scriptsize$\pm$9.8} & \textbf{59.0}\,{\scriptsize$\pm$4.0} & 30.1\,{\scriptsize$\pm$3.3} & 14.8\,{\scriptsize$\pm$1.2} & 9.0\,{\scriptsize$\pm$1.5} \\
PAIRED & 81.7\,{\scriptsize$\pm$2.0} & 50.4\,{\scriptsize$\pm$1.2} & 28.9\,{\scriptsize$\pm$0.9} & 37.3\,{\scriptsize$\pm$1.9} & 11.3\,{\scriptsize$\pm$7.4} & 10.0\,{\scriptsize$\pm$8.0} & 23.0\,{\scriptsize$\pm$0.9} & 27.1\,{\scriptsize$\pm$1.8} & \textbf{17.6}\,{\scriptsize$\pm$0.5} & 14.9\,{\scriptsize$\pm$1.7} \\
PAIRED+UniBC & 80.5\,{\scriptsize$\pm$2.5} & 49.5\,{\scriptsize$\pm$2.5} & 29.5\,{\scriptsize$\pm$0.6} & 37.2\,{\scriptsize$\pm$0.8} & 10.0\,{\scriptsize$\pm$4.5} & 7.8\,{\scriptsize$\pm$4.1} & 24.0\,{\scriptsize$\pm$0.9} & 26.7\,{\scriptsize$\pm$3.8} & 17.1\,{\scriptsize$\pm$0.3} & 14.7\,{\scriptsize$\pm$1.5} \\
PAIRED+BiBC & \textbf{70.3}\,{\scriptsize$\pm$26.4} & 39.9\,{\scriptsize$\pm$15.3} & 24.6\,{\scriptsize$\pm$1.3} & 21.1\,{\scriptsize$\pm$1.6} & 0.2\,{\scriptsize$\pm$0.2} & 0.1\,{\scriptsize$\pm$0.1} & 27.4\,{\scriptsize$\pm$1.7} & 35.2\,{\scriptsize$\pm$2.2} & \textbf{17.9}\,{\scriptsize$\pm$0.3} & \textbf{23.2}\,{\scriptsize$\pm$1.6} \\
PAIRED+Evo & 89.2\,{\scriptsize$\pm$1.3} & \textbf{58.4}\,{\scriptsize$\pm$1.2} & 33.3\,{\scriptsize$\pm$3.7} & 40.7\,{\scriptsize$\pm$2.0} & 26.3\,{\scriptsize$\pm$4.9} & 29.6\,{\scriptsize$\pm$1.3} & 25.4\,{\scriptsize$\pm$2.2} & 32.2\,{\scriptsize$\pm$7.8} & \textbf{17.1}\,{\scriptsize$\pm$1.0} & \textbf{21.0}\,{\scriptsize$\pm$2.1} \\
\bottomrule
\end{tabular}


==> tables/stats.tex <==
\begin{tabular}{lcc}
\toprule
Method & IQM $d{=}0.25$ & IQM OOD suite \\
\midrule
DR & 0.32\,{\scriptsize[0.23, 0.39]} & 0.33\,{\scriptsize[0.25, 0.41]} \\
DR-easy & 0.92\,{\scriptsize[0.90, 0.95]} & 0.57\,{\scriptsize[0.54, 0.61]} \\
DR-mixed & 0.74\,{\scriptsize[0.71, 0.77]} & 0.75\,{\scriptsize[0.71, 0.79]} \\
Terrain-CL & 0.92\,{\scriptsize[0.87, 0.97]} & 0.89\,{\scriptsize[0.85, 0.94]} \\
PLR$^{\perp}$ & 0.55\,{\scriptsize[0.50, 0.59]} & 0.69\,{\scriptsize[0.63, 0.73]} \\
SFL & 0.62\,{\scriptsize[0.53, 0.71]} & 0.84\,{\scriptsize[0.75, 0.88]} \\
ACCEL & 0.87\,{\scriptsize[0.81, 0.91]} & 0.87\,{\scriptsize[0.84, 0.89]} \\
ACCEL-grow & 0.74\,{\scriptsize[0.71, 0.78]} & 0.82\,{\scriptsize[0.78, 0.86]} \\
ACCEL-SFL & 0.78\,{\scriptsize[0.71, 0.85]} & 0.71\,{\scriptsize[0.63, 0.79]} \\
ACCEL-LP & 0.94\,{\scriptsize[0.84, 0.97]} & 0.61\,{\scriptsize[0.50, 0.68]} \\
PAIRED & 0.32\,{\scriptsize[0.26, 0.40]} & 0.45\,{\scriptsize[0.39, 0.51]} \\
PAIRED+UniBC & 0.29\,{\scriptsize[0.25, 0.34]} & 0.41\,{\scriptsize[0.36, 0.47]} \\
PAIRED+BiBC & 0.18\,{\scriptsize[0.10, 0.26]} & 0.28\,{\scriptsize[0.21, 0.37]} \\
PAIRED+Evo & 0.56\,{\scriptsize[0.50, 0.64]} & 0.86\,{\scriptsize[0.81, 0.90]} \\
\bottomrule
\end{tabular}


==> tables/uniform.tex <==
\begin{tabular}{llccc}
\toprule
Robot & Method & Uniform & CVaR$_{25}$ & Solvable \\
\midrule
W01-TEK & DR & 36.0\,{\scriptsize$\pm$2.0} & 16.0\,{\scriptsize$\pm$1.3} & 36.9\,{\scriptsize$\pm$2.0} \\
 & DR-easy & 37.8\,{\scriptsize$\pm$0.7} & 17.2\,{\scriptsize$\pm$0.6} & 38.8\,{\scriptsize$\pm$0.7} \\
 & DR-mixed & \textbf{42.2}\,{\scriptsize$\pm$2.0} & \textbf{22.6}\,{\scriptsize$\pm$1.9} & \textbf{43.2}\,{\scriptsize$\pm$2.0} \\
 & Terrain-CL & \textbf{43.5}\,{\scriptsize$\pm$1.6} & \textbf{24.6}\,{\scriptsize$\pm$0.7} & \textbf{44.4}\,{\scriptsize$\pm$1.7} \\
 & PLR$^{\perp}$ & 38.1\,{\scriptsize$\pm$2.4} & 18.2\,{\scriptsize$\pm$2.0} & 39.0\,{\scriptsize$\pm$2.5} \\
 & SFL & 40.3\,{\scriptsize$\pm$1.1} & 18.3\,{\scriptsize$\pm$0.8} & 41.2\,{\scriptsize$\pm$1.1} \\
 & ACCEL & 39.5\,{\scriptsize$\pm$1.2} & 19.9\,{\scriptsize$\pm$1.5} & 40.4\,{\scriptsize$\pm$1.2} \\
 & ACCEL-grow & \textbf{42.2}\,{\scriptsize$\pm$3.5} & \textbf{23.6}\,{\scriptsize$\pm$3.7} & \textbf{43.1}\,{\scriptsize$\pm$3.5} \\
 & ACCEL-SFL & 40.5\,{\scriptsize$\pm$1.5} & \textbf{23.6}\,{\scriptsize$\pm$1.9} & 41.3\,{\scriptsize$\pm$1.6} \\
 & ACCEL-LP & 36.8\,{\scriptsize$\pm$1.5} & 17.3\,{\scriptsize$\pm$0.7} & 37.7\,{\scriptsize$\pm$1.5} \\
 & PAIRED & 36.4\,{\scriptsize$\pm$0.9} & 15.8\,{\scriptsize$\pm$0.7} & 37.2\,{\scriptsize$\pm$0.9} \\
 & PAIRED+UniBC & 36.3\,{\scriptsize$\pm$1.9} & 15.7\,{\scriptsize$\pm$1.2} & 37.1\,{\scriptsize$\pm$1.9} \\
 & PAIRED+BiBC & \textbf{27.9}\,{\scriptsize$\pm$14.1} & 11.0\,{\scriptsize$\pm$5.0} & \textbf{28.6}\,{\scriptsize$\pm$14.4} \\
 & PAIRED+Evo & \textbf{41.8}\,{\scriptsize$\pm$2.5} & \textbf{23.5}\,{\scriptsize$\pm$3.5} & \textbf{42.7}\,{\scriptsize$\pm$2.6} \\
\midrule
Go1 & DR & 3.9\,{\scriptsize$\pm$1.0} & 2.1\,{\scriptsize$\pm$0.3} & 4.5\,{\scriptsize$\pm$1.1} \\
 & DR-easy & 13.2\,{\scriptsize$\pm$1.5} & 6.7\,{\scriptsize$\pm$0.9} & 14.9\,{\scriptsize$\pm$1.7} \\
 & DR-mixed & 15.8\,{\scriptsize$\pm$2.2} & 8.0\,{\scriptsize$\pm$1.0} & 17.7\,{\scriptsize$\pm$2.4} \\
 & Terrain-CL & \textbf{19.1}\,{\scriptsize$\pm$1.9} & \textbf{9.9}\,{\scriptsize$\pm$0.7} & \textbf{21.4}\,{\scriptsize$\pm$2.2} \\
 & PLR$^{\perp}$ & 8.3\,{\scriptsize$\pm$1.6} & 4.0\,{\scriptsize$\pm$1.1} & 9.4\,{\scriptsize$\pm$1.8} \\
 & SFL & 10.3\,{\scriptsize$\pm$2.9} & 5.5\,{\scriptsize$\pm$1.9} & 11.6\,{\scriptsize$\pm$3.3} \\
 & ACCEL & \textbf{16.0}\,{\scriptsize$\pm$3.2} & \textbf{8.0}\,{\scriptsize$\pm$1.7} & \textbf{18.0}\,{\scriptsize$\pm$3.6} \\
 & ACCEL-grow & 10.7\,{\scriptsize$\pm$1.2} & 5.7\,{\scriptsize$\pm$0.6} & 12.0\,{\scriptsize$\pm$1.3} \\
 & ACCEL-SFL & 15.4\,{\scriptsize$\pm$2.1} & 7.9\,{\scriptsize$\pm$1.2} & 17.3\,{\scriptsize$\pm$2.3} \\
 & ACCEL-LP & \textbf{17.5}\,{\scriptsize$\pm$2.6} & \textbf{8.6}\,{\scriptsize$\pm$1.4} & \textbf{19.6}\,{\scriptsize$\pm$2.9} \\
 & PAIRED & 4.1\,{\scriptsize$\pm$0.2} & 2.0\,{\scriptsize$\pm$0.1} & 4.6\,{\scriptsize$\pm$0.2} \\
 & PAIRED+UniBC & 4.1\,{\scriptsize$\pm$0.1} & 1.9\,{\scriptsize$\pm$0.1} & 4.7\,{\scriptsize$\pm$0.1} \\
 & PAIRED+BiBC & 4.4\,{\scriptsize$\pm$0.6} & 2.9\,{\scriptsize$\pm$0.7} & 5.0\,{\scriptsize$\pm$0.7} \\
 & PAIRED+Evo & 5.7\,{\scriptsize$\pm$0.5} & 2.7\,{\scriptsize$\pm$0.4} & 6.5\,{\scriptsize$\pm$0.5} \\
\midrule
Go2 & DR & 1.5\,{\scriptsize$\pm$0.7} & 1.0\,{\scriptsize$\pm$0.4} & 3.1\,{\scriptsize$\pm$1.4} \\
 & DR-easy & 2.3\,{\scriptsize$\pm$0.7} & 1.2\,{\scriptsize$\pm$0.3} & 4.5\,{\scriptsize$\pm$1.3} \\
 & DR-mixed & 2.2\,{\scriptsize$\pm$0.3} & 1.2\,{\scriptsize$\pm$0.3} & 4.5\,{\scriptsize$\pm$0.6} \\
 & Terrain-CL & \textbf{3.0}\,{\scriptsize$\pm$1.1} & \textbf{1.6}\,{\scriptsize$\pm$0.4} & \textbf{5.9}\,{\scriptsize$\pm$2.1} \\
 & PLR$^{\perp}$ & 1.8\,{\scriptsize$\pm$0.2} & 1.1\,{\scriptsize$\pm$0.1} & 3.6\,{\scriptsize$\pm$0.5} \\
 & SFL & 2.4\,{\scriptsize$\pm$1.3} & \textbf{1.4}\,{\scriptsize$\pm$0.7} & 4.8\,{\scriptsize$\pm$2.5} \\
 & ACCEL & \textbf{4.4}\,{\scriptsize$\pm$1.0} & \textbf{2.1}\,{\scriptsize$\pm$0.5} & \textbf{8.6}\,{\scriptsize$\pm$1.8} \\
 & ACCEL-grow & 2.2\,{\scriptsize$\pm$0.4} & 1.2\,{\scriptsize$\pm$0.2} & 4.4\,{\scriptsize$\pm$0.7} \\
 & ACCEL-SFL & 2.1\,{\scriptsize$\pm$1.0} & 1.1\,{\scriptsize$\pm$0.3} & 4.3\,{\scriptsize$\pm$2.0} \\
 & ACCEL-LP & 2.5\,{\scriptsize$\pm$1.2} & \textbf{1.5}\,{\scriptsize$\pm$0.6} & 4.8\,{\scriptsize$\pm$2.3} \\
 & PAIRED & 1.0\,{\scriptsize$\pm$0.8} & 0.7\,{\scriptsize$\pm$0.5} & 2.1\,{\scriptsize$\pm$1.6} \\
 & PAIRED+UniBC & 0.7\,{\scriptsize$\pm$0.5} & 0.5\,{\scriptsize$\pm$0.3} & 1.4\,{\scriptsize$\pm$1.0} \\
 & PAIRED+BiBC & 0.0\,{\scriptsize$\pm$0.0} & 0.0\,{\scriptsize$\pm$0.0} & 0.0\,{\scriptsize$\pm$0.0} \\
 & PAIRED+Evo & 2.9\,{\scriptsize$\pm$0.7} & \textbf{1.5}\,{\scriptsize$\pm$0.3} & 5.8\,{\scriptsize$\pm$1.3} \\
\midrule
Barkour vB & DR & 1.0\,{\scriptsize$\pm$0.0} & 0.7\,{\scriptsize$\pm$0.1} & 1.8\,{\scriptsize$\pm$0.1} \\
 & DR-easy & 2.4\,{\scriptsize$\pm$0.4} & 1.2\,{\scriptsize$\pm$0.1} & 4.3\,{\scriptsize$\pm$0.7} \\
 & DR-mixed & 2.3\,{\scriptsize$\pm$0.4} & 1.2\,{\scriptsize$\pm$0.3} & 4.2\,{\scriptsize$\pm$0.7} \\
 & Terrain-CL & \textbf{5.0}\,{\scriptsize$\pm$0.4} & \textbf{2.3}\,{\scriptsize$\pm$0.4} & \textbf{8.8}\,{\scriptsize$\pm$0.8} \\
 & PLR$^{\perp}$ & 2.6\,{\scriptsize$\pm$0.6} & 1.4\,{\scriptsize$\pm$0.3} & 4.7\,{\scriptsize$\pm$1.0} \\
 & SFL & 3.1\,{\scriptsize$\pm$0.2} & 1.6\,{\scriptsize$\pm$0.1} & 5.7\,{\scriptsize$\pm$0.4} \\
 & ACCEL & 4.0\,{\scriptsize$\pm$0.4} & \textbf{1.9}\,{\scriptsize$\pm$0.3} & 7.1\,{\scriptsize$\pm$0.6} \\
 & ACCEL-grow & 4.1\,{\scriptsize$\pm$0.4} & \textbf{2.0}\,{\scriptsize$\pm$0.2} & 7.4\,{\scriptsize$\pm$0.7} \\
 & ACCEL-SFL & 3.8\,{\scriptsize$\pm$0.8} & \textbf{1.8}\,{\scriptsize$\pm$0.4} & 6.8\,{\scriptsize$\pm$1.4} \\
 & ACCEL-LP & 2.7\,{\scriptsize$\pm$0.6} & 1.3\,{\scriptsize$\pm$0.1} & 4.9\,{\scriptsize$\pm$1.1} \\
 & PAIRED & 1.2\,{\scriptsize$\pm$0.3} & 0.7\,{\scriptsize$\pm$0.3} & 2.3\,{\scriptsize$\pm$0.5} \\
 & PAIRED+UniBC & 1.2\,{\scriptsize$\pm$0.2} & 0.6\,{\scriptsize$\pm$0.2} & 2.2\,{\scriptsize$\pm$0.3} \\
 & PAIRED+BiBC & 2.2\,{\scriptsize$\pm$0.2} & 1.4\,{\scriptsize$\pm$0.3} & 4.0\,{\scriptsize$\pm$0.4} \\
 & PAIRED+Evo & 1.6\,{\scriptsize$\pm$0.9} & 0.8\,{\scriptsize$\pm$0.3} & 2.9\,{\scriptsize$\pm$1.6} \\
\midrule
Spot & DR & 0.2\,{\scriptsize$\pm$0.1} & 0.2\,{\scriptsize$\pm$0.1} & 1.7\,{\scriptsize$\pm$0.4} \\
 & DR-easy & 0.1\,{\scriptsize$\pm$0.0} & 0.1\,{\scriptsize$\pm$0.0} & 1.0\,{\scriptsize$\pm$0.1} \\
 & DR-mixed & 0.3\,{\scriptsize$\pm$0.0} & 0.2\,{\scriptsize$\pm$0.0} & 2.1\,{\scriptsize$\pm$0.3} \\
 & Terrain-CL & 0.2\,{\scriptsize$\pm$0.0} & 0.2\,{\scriptsize$\pm$0.1} & 1.9\,{\scriptsize$\pm$0.3} \\
 & PLR$^{\perp}$ & 0.2\,{\scriptsize$\pm$0.0} & 0.2\,{\scriptsize$\pm$0.1} & 1.7\,{\scriptsize$\pm$0.3} \\
 & SFL & 0.4\,{\scriptsize$\pm$0.1} & 0.3\,{\scriptsize$\pm$0.0} & 2.9\,{\scriptsize$\pm$0.4} \\
 & ACCEL & 0.5\,{\scriptsize$\pm$0.1} & 0.4\,{\scriptsize$\pm$0.1} & 4.0\,{\scriptsize$\pm$0.5} \\
 & ACCEL-grow & 0.4\,{\scriptsize$\pm$0.1} & 0.3\,{\scriptsize$\pm$0.1} & 2.8\,{\scriptsize$\pm$0.8} \\
 & ACCEL-SFL & 0.4\,{\scriptsize$\pm$0.1} & 0.3\,{\scriptsize$\pm$0.1} & 2.8\,{\scriptsize$\pm$0.5} \\
 & ACCEL-LP & 0.1\,{\scriptsize$\pm$0.0} & 0.1\,{\scriptsize$\pm$0.0} & 1.0\,{\scriptsize$\pm$0.2} \\
 & PAIRED & 0.5\,{\scriptsize$\pm$0.1} & 0.3\,{\scriptsize$\pm$0.0} & 3.6\,{\scriptsize$\pm$0.7} \\
 & PAIRED+UniBC & 0.5\,{\scriptsize$\pm$0.1} & 0.4\,{\scriptsize$\pm$0.1} & 3.8\,{\scriptsize$\pm$0.7} \\
 & PAIRED+BiBC & \textbf{1.1}\,{\scriptsize$\pm$0.2} & \textbf{0.7}\,{\scriptsize$\pm$0.2} & \textbf{7.9}\,{\scriptsize$\pm$0.9} \\
 & PAIRED+Evo & 0.8\,{\scriptsize$\pm$0.1} & \textbf{0.6}\,{\scriptsize$\pm$0.1} & 5.3\,{\scriptsize$\pm$0.5} \\
\bottomrule
\end{tabular}

